TV-based Spline Reconstruction with Fourier Measurements: Uniqueness and Convergence of Grid-Based Methods

We study the problem of recovering piecewise-polynomial periodic functions from their low-frequency information. This means that we only have access to possibly corrupted versions of the Fourier samples of the ground truth up to a maximum cutoff frequency $K_c$. The reconstruction task is specified as an optimization problem with total-variation (TV) regularization (in the sense of measures) involving the $M$-th order derivative regularization operator $\mathrm{L} = \mathrm{D}^M$. The order $M \geq 1$ determines the degree of the reconstructed piecewise polynomial spline, whereas the TV regularization norm, which is known to promote sparsity, guarantees a small number of pieces. We show that the solution of our optimization problem is always unique, which, to the best of our knowledge, is a first for TV-based problems. Moreover, we show that this solution is a periodic spline matched to the regularization operator $\mathrm{L}$ whose number of knots is upper-bounded by $2 K_c$. We then consider the grid-based discretization of our optimization problem in the space of uniform $\mathrm{L}$-splines. On the theoretical side, we show that any sequence of solutions of the discretized problem converges uniformly to the unique solution of the gridless problem as the grid size vanishes. Finally, on the algorithmic side, we propose a B-spline-based algorithm to solve the grid-based problem, and we demonstrate its numerical feasibility experimentally. On both of these aspects, we leverage the uniqueness of the solution of the original problem.

==> sections/sec-algo.tex <==
% !TEX root = ../main.tex

%
\section{Frank-Wolfe Algorithm for Periodic Spline Reconstruction}\label{sec:algo}

In this section we propose a novel algorithm based on the Frank-Wolfe algorithm~\cite{Frank1956algorithm}, which solves the following optimization problem
\begin{align}\label{eq:optimpb-fw}
\mathcal{V}_{\lambda}(\bm{y}) =	\underset{f\in\ML}{\arg \min} \ \frac{1}{2} \norm{\bm{y} - \nuf(f) }_2^2 + \la\mnorm{\Op L f}
\end{align}
for elliptic operators $\Lop$ and where $\lVert \bm{y} - \bm{\nu}(f) \rVert_2^2 = \sum_{k=0}^{K_c} |y_k - \widehat{f}[k]|^2$. 
It is inspired from the Sliding Frank-Wolfe algorithm~\cite{denoyelle2019sliding}, but requires several non-trivial adaptations, due to the nature of our problem~\eqref{eq:optimpb-fw}, that we detail in Section~\ref{subsec:presentation-algo}. In Section~\ref{subsec:convergence-algo}, we prove that it recovers the unique solution of problem~\eqref{eq:optimpb-fw} in a finite number of main steps. % under a mild non-degeneracy assumption.
%Finally in Section~\ref{subsec:numerical-xp}, we provide some numerical experiments.

\textit{Remark.} We may consider non-quadratic data-fidelity cost functional $E$ in \eqref{eq:optimpb-fw}: the Frank-Wolfe machinery simply requires that $E$ is differentiable and gradient Lipschitz. We present this case for the sake of simplicity. Note that the quadratic data-fidelity clearly satisfies the assumption of Proposition~\ref{prop:y0forz0}, hence for any $f^*$ solution of \eqref{eq:optimpb-fw}, $\widehat{f}^*[0] = y_0$. 

%
\subsection{Presentation of the Algorithm}\label{subsec:presentation-algo}

We recall that the Frank-Wolfe algorithm, introduced by Frank and Wolfe in 1956~\cite{Frank1956algorithm}, is tailored to solving optimization problems of the form
\begin{align}\label{eq:minfw}
\min_{m \in C}\ f(m),
\end{align}
where $C$ is a weakly compact convex set of a Banach space, and $f$ is a differentiable convex function. It does not appear at first sight that we can use this algorithm for our problem since the search space is not bounded and the objective function is non differentiable due to the total-variation norm. Let us first prove, in the following Lemma, that problem~\eqref{eq:optimpb-fw} can be recast into the proper form by using an epigraphical lift.

%
\begin{lemma}\label{lem:equivalent-optimpb}
The function $f^*\in\ML$ is a solution of problem~\eqref{eq:optimpb-fw} if and only if $(w^*,t^*)\in\RadonO\times\RR^+$, given through the unique decomposition (see \eqref{eq:uniquedecompo})
\begin{align}\label{eq:link-equi-fw}
	f^* = \Lop^{\dagger} w^* + y_0,
\end{align}
is a solution of
\begin{align}\label{eq:optimpb-fw-equi}
	\underset{\underset{\mnorm{w}\leq t \leq M}{(w,t)\in\RadonO\times\RR^+}}{\min} \ \frac{1}{2} \norm{\tilde{\bm{y}} - \num(w)}_2^2 + \la t,
\end{align}
where $\tilde{\bm{y}}\in\R^+\times \C^{K_c}$ is such that
$\tilde{y}_k={y}_k$ for every $1 \leq k \leq K_c$ and $\tilde{y}_0=0$, 
%\quentin{vérifier indexation des vecteurs}
and $M = M(\tilde{\bm{y}}, \lambda) = \frac{\norm{\tilde{\bm{y}}}_2^2}{2\lambda}$. Moreover, we have $t^*=\mnorm{w^*}$.

The search space of the equivalent problem~\eqref{eq:optimpb-fw-equi}, denoted by $C=\{(w,t)\in\RadonO\times\RR^+; \ \mnorm{w}\leq t \leq M\}$ is a weak*-compact convex subset of $\RadonO\times\RR^+$. Its objective function, denoted by $T_\lambda$, is differentiable and its differential at any $(w,t)\in\RadonO\times\RR^+$ is given by
\begin{align}\label{eq:differential:objfunc}
 \forall (\tilde w, \tilde t)\in\RadonO\times\RR^+, \quad \mathrm{d} T_\lambda(w,t)\cdot (\tilde w, \tilde t) = \dotp{\tilde w}{\num^*(\num(w) - \tilde{\bm{y}})} + \la \tilde t.
\end{align}
Moreover, $\mathrm{d} T_\la$ is Lipschitz continuous.
\end{lemma}
%

%
\begin{proof}
Due to Lemma \ref{lemma:quasilemma} applied to the penalized problem~\eqref{eq:optimpb-fw}, we have $f^*\in \mathcal{V}_{\lambda}(\bm{y})$ if and only if $w^* = \Lop^\dagger f^* \in\RadonO$ is a solution of
\begin{align}\label{eq:gBLASSO-equi}
	\underset{w\in\RadonO}{\min} \ \frac{1}{2} \norm{\num(w) - \tilde{\bm{y}}}_2^2 + \la\mnorm{w},
\end{align}
with $\bm{\nu}_{\Lop} =\nuf\circ\Lop^\dagger:\RadonO\to\R \times \C^{K_c}$. 
%$\num=\nuf\circ\Lop^\dagger:\RadonO\to\R \times \C^{K_c}$. 
%and $\tilde{\bm{y}}\in\CC^M$ such that
%\eq{
%	\forall m\neq 0, \ \tilde{\bm{y}}[m]=\bm{y}[m] \qandq \tilde{\bm{y}}[0]=0
%}

Now, evaluating the objection function of problem~\eqref{eq:gBLASSO-equi} at $w=0$ shows that any solution $w^*$ of~\eqref{eq:gBLASSO-equi} must satisfy $\mnorm{w^*}\leq M = \frac{\norm{y}^2_2}{2\la}$. Finally, we obtain~\eqref{eq:optimpb-fw-equi} by using an epigraph representation.

The differential of the objective function $T_\la$ is easily obtained and is Lipschitz continuous since
\eq{
	\mathrm{d} T_\la(w,t) - \mathrm{d} T_\la(w',t') = (\bm{\nu}_{\Lop}^*\circ \bm{\nu}_{\Lop} ) (w - w'),
}
and $\bm{\nu}_{\Lop}^*\circ \bm{\nu}_{\Lop} : \RadonO \to \Cc(\TT)$ is a continuous linear operator as a combination of four continuous and linear operators. 
%\quentin{continue pour la topologie forte?}
\end{proof}

The Frank-Wolfe algorithm can therefore be applied to problem~\eqref{eq:optimpb-fw-equi}. It directly provides a solution of problem~\eqref{eq:gBLASSO-equi}, but also of~\eqref{eq:optimpb-fw} thanks to the bijection given in~\eqref{eq:link-equi-fw}. This algorithm, also known as the Conditional Gradient Method (CGM), is recalled in Algorithm~\ref{alg:fw} in our setup (problem~\eqref{eq:optimpb-fw-equi}).

\begin{algorithm}
    \caption{Frank-Wolfe Algorithm for Problem~\eqref{eq:optimpb-fw-equi}}
    \label{alg:fw}
    \begin{algorithmic}[1]
    \State $w^{[0]} = 0$
    \For{$k=0,\ldots, n$}
    \State\label{fw-greedy-step}Minimize: $(\iter{\tilde{w}}, \iter{\tilde{t}})\in \mbox{argmin}_{(\tilde{w},\tilde t)\in C} \ T_\lambda(\iter{w},\iter{t})+dT_\lambda(\iter{w},\iter{t})[(\tilde{w},\tilde t)-(\iter{w},\iter{t})]$
    \If{$dT_\lambda(\iter{w},\iter{t})[(\iter{\tilde{w}}, \iter{\tilde{t}})-(\iter{w},\iter{t})]=0$}\label{stopping-conditionFW}
       \State \Return $(\iter{w},\iter{t})$
    \Else{}
    \State\label{fw-stepresearch} Line search: $\iter{\ga}\gets \frac{2}{k+2}$ or $\iter{\ga}\in \mbox{argmin}_{\gamma\in [0,1]} T_\lambda(\iter{w},\iter{t})+\gamma((\iter{\tilde{w}}, \iter{\tilde{t}})-(\iter{w},\iter{t})))$
    \State\label{fw-tentativeupdate} Update: $(\iterpo{w},\iterpo{t})\gets (\iter{w},\iter{t})+\iter{\ga}((\iter{\tilde{w}}, \iter{\tilde{t}})-(\iter{w},\iter{t}))$
%    \State\label{fw-tentativeupdate} Tentative update: $\tilde{m}_{k+1}\gets (\iter{w},\iter{t})+\iter{\ga}(s-(\iter{w},\iter{t}))$. 
%    \State\label{fw-final-update} Final update: $\iterpo{m}\gets \tilde{m}_{k+1}$ or $\iterpo{m}\gets x\in C$ with $T_\lambda(x)\leq T_\lambda(\tilde{m}_{k+1})$.
    \EndIf
    \EndFor
    \end{algorithmic}
\end{algorithm}

Note that Algorithm~\ref{alg:fw} only requires the computations of directional derivatives and the ability to minimize a linear form over the weak*-compact convex set $C$. Let us take a deeper look at this step~\ref{fw-greedy-step}. As it consists in minimizing a continuous linear form over a weak*-compact convex set, there exists at least one extreme point of $C$ that is solution. In the case of the Sliding Frank-Wolfe algorithm presented in~\cite{denoyelle2019sliding}, the extreme points of $C$ involve those of the unit ball of the space of Radon measures, which are well known to be Dirac masses. This is a key difference with our paper since here the measure part of $C$ is restricted to the Banach subspace of Radon measures with zero mean $\RadonO$. As a result, Step~\ref{fw-greedy-step} is different in our setup. This is summarized in the next Lemma.

\begin{lemma}\label{lem:greedy}
Step~\ref{fw-greedy-step} can be equivalently formulated as the following procedure:
\begin{enumerate}
\item solve 
\begin{align}
	\tilde x \in \mbox{argmax}_{x\in\TT} \ \iter{\eta}(x) \qandq \tilde y \in \mbox{argmin}_{y\in\TT} \ \iter{\eta}(y),
\end{align}
with $\iter{\eta} = \frac{1}{\la}\num^*(\tilde{\bm{y}}-\num(\iter{w}))\in\Cc(\TT)$
\item if $\iter{\eta}(\tilde x) - \iter{\eta}(\tilde y) \geq 2$, then take $(\iter{\tilde{w}}, \iter{\tilde{t}})=(\frac{M}{2}(\dirac{\tilde x}-\dirac{\tilde y}), M)$ as a solution of step~\ref{fw-greedy-step},
\item otherwise, take $(\iter{\tilde{w}}, \iter{\tilde{t}})=(0,0)$.
\end{enumerate}
\end{lemma}

\begin{proof}
As mentioned before, we know that there is at least one extreme point of $C$ which minimizes the continuous linear form
\eq{
	(\tilde{w},\tilde t)\mapsto dT_\lambda(\iter{w},\iter{t})\cdot(\tilde{w},\tilde t),
}
\ie that provides a solution for Step~\ref{fw-greedy-step}. By Equation~\eqref{eq:differential:objfunc}, such an extreme point equivalently maximizes
\begin{align}\label{eq:greedy-eq}
	R_\lambda:(\tilde{w},\tilde t)\mapsto \dotp{\tilde w}{\frac{1}{\la}\num^*(\tilde{\bm{y}} - \num(\iter{w}))} - \tilde t.
\end{align}

The extreme points of $C$ are given by 
\begin{equation}
    \{ (0,0)\} \cup \left\{ \left( \frac{M}{2}(\dirac{x} - \dirac{y}), M \right), \ (x,y)\in\TT^2 \right\},
\end{equation}
since the extreme points of the unit ball for the total-variation norm in $\RadonO$ are the $\frac{1}{2}(\dirac{x} - \dirac{y})$ as stated in Proposition~\ref{prop:extremePointsB0} in Appendix~\ref{appendix:extremepoints-M0}.

Therefore, verifying whether some $(\tilde{w},\tilde t)=(\frac{M}{2}(\dirac{\tilde x} - \dirac{\tilde y}), M)$ with $\tilde x,\tilde y\in\TT$ is an extreme points of $C$ solution of~\eqref{eq:greedy-eq}, amounts to:
\begin{itemize}
\item solve $\mbox{argmax}_{(x,y)\in\TT^2} \ \frac{1}{2}(\iter{\eta}(x)-\iter{\eta}(y)) - 1$ where $\iter{\eta} = \frac{1}{\la}\num^*(\tilde{\bm{y}} - \num(\iter{w}))$ or equivalently
\eq{
	\tilde x \in\mbox{argmax}_{x\in\TT} \ \iter{\eta}(x) \qandq \tilde y \in\mbox{argmin}_{y\in\TT} \ \iter{\eta}(y),
}
\item then check if
\eq{
	\iter{\eta}(\tilde x) - \iter{\eta}(\tilde y) \geq 2,
}
\item otherwise, if $\iter{\eta}(\tilde x) - \iter{\eta}(\tilde y) < 2$, then $\max_{(x,y)\in\TT^2} \ \frac{1}{2}(\iter{\eta}(x)-\iter{\eta}(y)) - 1 < 0$ which means that the only extreme-point solution of~\eqref{eq:greedy-eq} is $(0,0)$ as $R_\lambda (0,0)=0$.
\end{itemize}

\end{proof}

From Lemma~\ref{lem:greedy}, we see that, fundamentally, the Frank-Wolfe algorithm applied to our problem consists in recursively adding pairs of Dirac masses located at the maximum and minimum of some continuous function $\iter{\eta}$. This is one of the main differences between our algorithm and the Sliding Frank-Wolfe algorithm where only one Dirac mass, located at the maximum of $\Vert \iter \eta \Vert_\infty$, was added at each iteration. It boils down to the fact that, in our setup, measures must have zero mean.

\textit{Remark.}
As noted in~\cite{denoyelle2019sliding}, it is possible to prove that the stopping criterion of the Frank-Wolfe algorithm in Step~\ref{stopping-conditionFW}, which is the standard one for constrained convex optimization problems, is in fact equivalent to the optimality conditions of Problem~\eqref{eq:gBLASSO-equi} which state that \quentin{le mettre quelque part?} $w^*\in\RadonO$ is the solution of~\eqref{eq:gBLASSO-equi} if and only if
\begin{align}
	\eta_\lambda = \frac{1}{\la}\num^*(\tilde{\bm{y}} - \num(w^*))\in\Cc(\TT) \text{ satisfies } \normv{\eta_\lambda} \leq 2,\\
	\text{ and } \ssupp{w^*}\subset \ssat{\eta_\lambda - \frac{1}{2}(\max \eta_\lambda + \min \eta_\lambda)}.
\end{align}
Note that $\Cc(\TT)$ is not endowed with the supremum norm $\normi{\cdot}$ but with the semi-norm $\normv{\cdot}=\max(\cdot)-\min(\cdot)$.


% Say that from now on we drop the t part.
% introduce sliding with the fact that FW allows to choose a better candidate in the end.
% Put the whole algorithm and explain: 1)why we don't need to consider (0,0) as extreme point in creation step (because the interpolation condition in OC is satisfied so ||\eta_k||_\Delta <=2 is enough as stopping criteria)







    
%%
\subsection{Convergence of the Algorithm}\label{subsec:convergence-algo}
    

%%
\subsection{Numerical Experiments}\label{subsec:numerical-xp}



